Towards Fault Localization via Probabilistic Software Modeling

Software testing helps developers to identify bugs. However, awareness of bugs is only the first step. Finding and correcting the faulty program components is equally hard and essential for high-quality software. Fault localization automatically pinpoints the location of an existing bug in a program. It is a hard problem, and existing methods are not yet precise enough for widespread industrial adoption. We propose fault localization via Probabilistic Software Modeling (PSM). PSM analyzes the structure and behavior of a program and synthesizes a network of Probabilistic Models (PMs). Each PM models a method with its inputs and outputs and is capable of evaluating the likelihood of runtime data. We use this likelihood evaluation to find fault locations and their impact on dependent code elements. Results indicate that PSM is a robust framework for accurate fault localization.

==> reviews.tex <==
1: (weak accept)
Paper Summary
----------------------------------
This paper investigates the usage of Probabilistic Software Modeling (PSM) for fault localization. More in details, the authors try to infer possible fault locations as well as their impact on dependent code elements. The application of the approach (i.e., FL-PSM) on the Nutrition Advisor example, on which the authors have injected two different types of fault (one unit and one integration fault), highlights that FL-PSM is able to detect faults as well as is able to properly visualize in a more-human format the regions in the program where the fault is more likely located.

General Evaluation
----------------------------------
The paper addresses a very hot topic in the field of Validation, Analysis and Evolution of Software Tests. However, it does not clarify very well how the network has been trained and, more importantly, the authors do not report how FL-PSM produce different (and probably better) results compared to state of the art approach like Tarantula or Ochiai. Moreover, it would be interesting to see the performance of FL-PSM while using some real cases extracted from the Defects4J dataset[a]. Another problem is related to the choice of using the Non-Volume Preserving Transformations as a neural network since it has been proven to work well while modelling natural images only.

Please consider my suggestions for extending the work in the future.

[a] R.Just and D.Jalali and M.D.Ernst, Defects4J: a database of existing faults to enable controlled testing studies for Java programs, In International Symposium on Software Testing and Analysis, {ISSTA}'14, San Jose, CA, {USA} - July 21 - 26, 2014.

Brief Summary
----------------------------------
- The topic of the paper matches the theme of the workshop.
- The paper, as is, has some potential to inspire interesting discussions when presented at the workshop.
- The submission meets standards for scientific publications and professional work.

------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

1: (weak accept)
This paper proposes to perform fault localization via Probabilistic Software Modeling (PSM), which uses the probabilistic models to build via PSM to infer possible fault locations as well as their impact on the dependent code elements.
Results indicate that PSM is a promising technique for fault localization

Fault localization approaches have been proposed in the last years and the authors of this paper propose to perform fault localization via Probabilistic Software Modeling (PSM). This is an interesting direction and I think is a valid and intuitive alternative to previous work. However, I think the paper should integrate a direct comparison with at least one baseline approach to show the relevance of the proposed approach.

Summary of points in favor and against:
+ Interesting and well-described idea
- missing comparison with a baseline approach to show the relevance of the proposed approach
- practical implications of using this approach compared to previous techniques unclear
- size of the study a bit small

------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

1: (weak accept)
Motivation: The topic of the paper does match the theme of the workshop, has potential to spark an interesting discussion. However, work is needed as it barely meets standards for scientific publication.


Summary
This paper proposes a variant of a fault localisation heuristic based on probabilistic software modelling. The authors demonstrate on a small yet representative case that the heuristic is able to localise non-trivial faults.


Strong points

+ The authors demonstrate the feasibility of probabilistic software models for fault localisation. Whether this heuristic is capable to complement existing fault localisation heuristics is an area for future work but for a position paper in a testing workshop this is good enough.

+ I appreciate the motivating example of the Nutrition Advisor. The injected faults are well-chosen. Fault one (replacing +weight with -weight) is a typical mutation fault; fault 2 (computing the body mass index in meters versus inches) reminded me of the fault that caused the mars orbiter crash.


Points that should be addressed

In its current form, the paper it barely meets standards for scientific publication. Here are a few issues that must be addressed in the camera ready version of the paper.

- Motivation. Better motivate why an alternative for spectrum based fault localisation is warranted. I would argue that your heuristic has the potential to complement existing heuristics. In particular it has the potential to deal with faults which are spread across multiple lines; traditionally a weak point of spectrum based fault localisation. Also it is likely to work better for difficult to localise faults revealed only by component tests. (See "Unit tests and component tests do make a difference on fault localisation effectiveness" - https://doi.org/10.1145/3183440.3194970)

- Unsupported claim (1). The authors argue that the visualisations allow for easy interpretation. (p. 3 - "The other important aspect is the visualization of detected faults (Figure 2 and 3) allowing for easy comprehension of results via humans. ") This is not supported by any evidence from actual user observations. Remove this claim from the paper.

- Unsupported claim (2) "FL-PSM is tailored for teams to be integrated into the continuous integration " This may be your goal but for the moment you don't have any evidence that supports this claim. Remove this claim from the paper.

- On p. the authors state "Figure 2 shows the runtime behavior of a subset of code". How is this subset selected? This is a crucial aspect as it immediately affects the visualisation which is an important feature of the heuristic.

- Avoid the use of acronyms. This makes the paper unnecessarily hard to read. "PM" for me is the acronym for "post meridiem"; PSM is an acronym used for "Professional Scrum Master" in Software Engineering Circles.


Minor details

- p.4 "while SBFL techniques work on a statement level." Spectrum based fault localisation has been shown to work on various granularity levels (statement / block/ function / …)
